3D Scene Grammar for Parsing RGB-D Pointclouds

We pose 3D scene-understanding as a problem of parsing in a grammar. A grammar helps us capture the compositional structure of real-word objects, e.g., a chair is composed of a seat, a back-rest and some legs. Having multiple rules for an object helps us capture structural variations in objects, e.g., a chair can optionally also have arm-rests. Finally, having rules to capture composition at different levels helps us formulate the entire scene-processing pipeline as a single problem of finding most likely parse-tree---small segments combine to form parts of objects, parts to objects and objects to a scene. We attach a generative probability model to our grammar by having a feature-dependent probability function for every rule. We evaluated it by extracting labels for every segment and comparing the results with the state-of-the-art segment-labeling algorithm. Our algorithm was outperformed by the state-or-the-art method. But, Our model can be trained very efficiently (within seconds), and it scales only linearly in with the number of rules in the grammar. Also, we think that this is an important problem for the 3D vision community. So, we are releasing our dataset and related code.

==> contextproperties.tex <==
\vspace*{\sectionReduceTop}
\section{Approach}\label{S.properties}
\vspace*{\sectionReduceBot}

We now outline our approach, including the model, its inference methods, and the learning algorithm. 
Our input is multiple Kinect RGB-D images of a scene (i.e., a room) stitched into a single 
3D point cloud using RGBDSLAM.\footnote{http://openslam.org/rgbdslam.html} Each such point cloud is 
then over-segmented based on smoothness (i.e., difference in the local surface normals) and 
continuity of surfaces  (i.e.,  distance between the points). These segments are the 
atomic units in our model. Our goal is to label each of them.
% segment.

% \todo{This section describes informally the general ideas that you are trying to capture.}

%  Our goal is to label each segment in the point-cloud. 
Before getting into the technical details of the model, the following outlines the properties we aim 
to capture in our model:

%There are several properties that help in the labeling the segments in a scene. They range from local shape and visual appearance properties to different types of ``contextual'' information.  In a scene, where the object itself may be quite small and can be fragmented into multiple segments, it is these contextual properties that often help in the correct labeling. In particular, we want to model the following properties:
%  in our work:
% of the segment that help in the detection
% of objects in a scene.

% the label of a segment is often determined
% by its relation to other parts in the scene. In particular, in our model we will
% model the following.
%   \todo{divide it into assoc and non-assoc}

% \begin{packed_item}
% This section should only be at a higher level and sort of motivate the model
% \item 
\noindent
\textbf{Visual appearance.} The reasonable success of object detection in 2D images 
shows that visual appearance is a good indicator for labeling scenes.
% of the segment label.
% valuable property for labeling a scene. 
We therefore model the local color, texture, gradients of intensities, etc.~for predicting the 
labels.
%  of a segment. 
In addition, we also model the property that if nearby segments are similar in 
visual appearance, they are more likely to belong to the same object.

% \item 
\noindent
\textbf{Local shape and geometry.}  Objects have characteristic 
shapes---for example, a table is horizontal, a monitor is vertical, a keyboard is uneven, 
and a sofa is usually smoothly curved. 
% Also, a monitor is always vertical, while a table is always horizontal. 
Furthermore, parts of an object often form a convex shape. We compute
3D shape features to capture this.

%\item
\noindent 
\textbf{Geometrical context.}
Many sets of objects occur in characteristic relative geometric configurations. 
For example, a monitor is always \emph{on-top-of} a table, chairs are usually found \emph{near} tables, a keyboard is \emph{in-front-of} a monitor.
% Unlike images, we can obtain precise information about relative position and orientation of objects in a pointcloud. 
This means that our model needs to capture non-associative relationships 
(i.e., that neighboring segments differ in their labels in specific patterns). 
%One important observation here is that objects in these relationships need not be the same. For example, we do not find a table above a table, but a monitor. In the terminology of Markov networks, the clique potentials capturing these properties need to be non-associative in nature. I.e., they can favor different labels for the neighboring nodes. Contrast this to the properties discussed earlier (e.g.~convexity, visual similarity)---which can be captured with clique potentials favoring same object-label. 

\smallskip
Note the examples given above are just illustrative. For any particular practical application, 
there will likely be other properties that could also be included. As demonstrated in the 
following section, our model is flexible enough to include a wide range of features.
% model
%that is not restricted to a few specifically designed properties, but one  
%that can learn such classes of properties from the labeled training data.
%  desining a learning
% algorithm is not to designis to design a learning
% algorithm that can 

\begin {comment}
\item \textbf{Visual appearance.}  We obtain the RGB values for the points in the segment. The
color and texture of a segment is often a good indicator of what object it is.  
% In order to capture the visual appearance of various objects we 
% use the commonly used features in computer vision.
We used histogram-of-gradients (HOG) features that have been successfully used in many object 
recognition tasks for images \cite{dalal2005histograms,felzenszwalb2008discriminatively}. 
% It is essentially a normalized histogram of intensity-gradient directions.  
We also compute average hue, saturation and intensity values of a segment and their histograms. 
% It is possible for the segmentation algorithm to segment one object into multiple segments. The similarity in the visual appearance of a pair of segments can be used to determine if they belong to the same object. For example, furniture such as tables and sofas have uniform color and texture. We compute the difference in average hue, saturation and intensity of the segments to model relative visual appearance.
\item \textbf{Local shape.}  Different objects have different shapes---for example, a table is flat while a keyboard
is uneven. We incorporate several shape properties based on surface normals, and other statistics
of the point-cloud in the segment. We describe these in Section~\ref{sec:features}.
%  shape properties such as the linear-ness, planar-ness, size, etc., of a segment play an important role in determining its label. 
\item \textbf{Co-occurence of the objects.}  Objects 
% like 
% ASHUTOSH: Do not use the work "like". Instead use "such as"
such as monitor and keyboard, or pillow and bed, usually co-occur. We need to capture these 
co-occurrence statistics in our model.
% the pair-wise potentials.
\item \textbf{Geometric properties.}  Certain objects follow strong relative location preferences,
% Relative geometric properties 
such as ``infront-of" or ``on-top-of" 
% can be useful in determining what the objects are. 
For example, a monitor is almost always \emph{on-top-of} 
a table and a keyboard is \emph{infront-of} a monitor.  
We model several geometric relations between a pair of
 segments:  relative depth-ordering (e.g., ``infront-of", ``behind"), relative horizontal-ordering 
 (``above", ``below" and ``same height"), coplanar-ness, etc.   See Section~\ref{sec:relfeatures}
 for more details.
% For any given pair of segments, the relative depth-ordering  captures the ``infront-of", ``behind" and 
% ``none" relations and the relative  horizontal-ordering captures the ``above", ``below" and ``same height" relations.
%\item \textbf{Convexity.} Convexity of the object is another important cue in determining the which segments belong to the same object. We also model this as a relative feature by checking if two adjacent segments  together have a convex shape.
\end{comment}

% \end{packed_item}





==> f1.tex <==
% Graphic for TeX using PGF
% Title: /Users/hema/Desktop/feats_f1.dia
% Creator: Dia v0.97.1
% CreationDate: Tue Oct 25 21:59:07 2011
% For: hema
% \usepackage{tikz}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pgf file will use them.
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{15\unitlength}
\begin{tikzpicture}
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathellipse{\pgfpoint{8.548942\du}{7.474961\du}}{\pgfpoint{1.003772\du}{0\du}}{\pgfpoint{0\du}{1.340521\du}}
\pgfusepath{fill}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathellipse{\pgfpoint{8.548942\du}{7.474961\du}}{\pgfpoint{1.003772\du}{0\du}}{\pgfpoint{0\du}{1.340521\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (8.548942\du,7.819405\du){$i$};
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfpathellipse{\pgfpoint{12.234809\du}{7.600002\du}}{\pgfpoint{1.019309\du}{0\du}}{\pgfpoint{0\du}{1.323252\du}}
\pgfusepath{fill}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\pgfpathellipse{\pgfpoint{12.234809\du}{7.600002\du}}{\pgfpoint{1.019309\du}{0\du}}{\pgfpoint{0\du}{1.323252\du}}
\pgfusepath{stroke}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (12.234809\du,7.944446\du){$j$};
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (1.150000\du,12.699900\du)--(5.700000\du,3.700000\du);
}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (5.700000\du,3.700000\du)--(18.300000\du,3.799930\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (8.200000\du,11.649900\du){};
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (5.118750\du,12.945800\du)--(5.118750\du,15.154133\du)--(8.081250\du,15.154133\du)--(8.081250\du,12.945800\du)--cycle;
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (5.118750\du,12.945800\du)--(5.118750\du,15.154133\du)--(8.081250\du,15.154133\du)--(8.081250\du,12.945800\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (6.600000\du,14.308300\du){cam};
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{to}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (6.600000\du,12.945800\du)--(8.164815\du,8.713441\du);
}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{to}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (8.933068\du,6.236481\du)--(9.850000\du,3.700000\du);
}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{to}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (6.600000\du,12.945800\du)--(11.293090\du,8.106388\du);
}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{to}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (12.850000\du,6.400000\du)--(15.400000\du,3.600000\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (4.700000\du,10.549900\du){$rh_i$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (6.749230\du,5.179110\du){$db_i$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (13.749200\du,6.129110\du){$db_j$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (8.999200\du,11.129100\du){$rh_j$};
\end{tikzpicture}


==> f2.tex <==
% Graphic for TeX using PGF
% Title: /Users/hema/Desktop/feats_f2.dia
% Creator: Dia v0.97.1
% CreationDate: Wed Oct 26 02:07:04 2011
% For: hema
% \usepackage{tikz}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pgf file will use them.
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{15\unitlength}
\begin{tikzpicture}
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (-1.424800\du,3.696728\du)--(8.625200\du,3.646728\du);
}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetdash{{1.000000\du}{1.000000\du}}{0\du}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (-1.274800\du,3.696728\du)--(-7.624800\du,-0.153272\du);
}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (-4.889800\du,7.131728\du)--(-4.889800\du,9.340061\du)--(-1.927300\du,9.340061\du)--(-1.927300\du,7.131728\du)--cycle;
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (-4.889800\du,7.131728\du)--(-4.889800\du,9.340061\du)--(-1.927300\du,9.340061\du)--(-1.927300\du,7.131728\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (-3.408550\du,8.494228\du){cam};
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{to}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (-3.408550\du,7.131728\du)--(-3.424800\du,2.396728\du);
}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{to}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (-3.408550\du,7.131728\du)--(1.525200\du,3.696728\du);
}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{to}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (-5.374800\du,1.346728\du)--(-6.724800\du,3.846728\du);
}
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{to}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (5.075200\du,3.746728\du)--(5.075200\du,6.596728\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (-5.174800\du,5.396728\du){$r_i$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (-0.724800\du,5.996728\du){$r_j$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (-7.874800\du,2.046728\du){$\hat{n}_i$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (5.425200\du,5.146728\du){$\hat{n}_j$};
\end{tikzpicture}


==> f3.tex <==
% Graphic for TeX using PGF
% Title: C:\Users\abhishek\Desktop\proj2\labeling3d\feat3.dia
% Creator: Dia v0.97.1
% CreationDate: Wed Oct 26 01:42:08 2011
% For: abhishek
% \usepackage{tikz}
% The following commands are not supported in PSTricks at present
% We define them conditionally, so when they are implemented,
% this pgf file will use them.
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{15\unitlength}
\begin{tikzpicture}
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (6.850000\du,6.700000\du)--(6.850000\du,9.850000\du)--(10.800000\du,9.850000\du)--(10.800000\du,6.700000\du)--cycle;
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetmiterjoin
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (6.850000\du,6.700000\du)--(6.850000\du,9.850000\du)--(10.800000\du,9.850000\du)--(10.800000\du,6.700000\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (8.825000\du,8.515000\du){i};
\pgfsetlinewidth{0.150000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetlinewidth{0.150000\du}
\pgfsetbuttcap
\pgfsetmiterjoin
\pgfsetdash{}{0pt}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\fill (15.200000\du,9.809822\du)--(22.000000\du,9.809822\du)--(18.600000\du,6.600000\du)--cycle;
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (15.200000\du,9.809822\du)--(22.000000\du,9.809822\du)--(18.600000\du,6.600000\du)--cycle;
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node at (18.600000\du,9.257367\du){};
\pgfsetlinewidth{0.100000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsstart{stealth}
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw (10.900000\du,9.450000\du)--(15.000000\du,9.400000\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (11.050000\du,10.400000\du){$dmin_{ij}$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (18.000000\du,8.604911\du){j};
\end{tikzpicture}


==> features.tex <==
% \vspace*{\subsectionReduceTop}
% \subsection{\label{sec:features}Features}
% \vspace*{\subsectionReduceBot}


\todo{[[Doesn't this section is exactly the same as the NIPS paper last year?]]}

Our features are same as \cite{abhishek_koppula:nips11}.



\iffalse
\begin{figure}[t!]
\vskip -.2in
\centering
%\includegraphics[width=.25\linewidth]{dbpc.pdf}
\includegraphics[width=.25\linewidth]{f1.pdf}
\hskip 0.1in
%\includegraphics[width=.25\linewidth]{normalpc.pdf}
\includegraphics[width=.25\linewidth]{f2.pdf}
\hskip 0.1in
%\includegraphics[width=.3\linewidth]{mindist.pdf}
\includegraphics[width=.3\linewidth]{f3.pdf}
\vspace*{\captionReduceTop}
\caption{{\small Illustration of a few features. (Left) Features N11 and E9. Segment i is infront of segment j if ${\bf rh_i }<{\bf rh_j}$. (Middle) Two connected segment i and j are form a convex shape if $(r_i-r_j).\hat{n_i} \ge 0$ and $(r_j-r_i).\hat{n_j} \ge 0$. (Right) Illustrating feature E8.} }
\label{fig:features}
\vspace*{\captionReduceBot}
\end{figure}

Table \ref{tab:Features}  summarizes the features used in our experiments. ${\lambda_i}_0,{\lambda_i}_1$ and ${\lambda_i}_2$ are the 3 eigen-values of the scatter matrix computed from the points of segment $i$ in decreasing order. 
%$s_i$ is the set of points in segment $i$.
$c_i$ is the centroid of  segment $i$. 
$r_i$ is the ray vector to the centroid of segment $i$ from the position camera in which it was captured. $rh_i$ is the projection of $r_i$ on horizontal plane. 
$\hat{n}_i$ is the unit normal of segment $i$ which points towards the camera ($r_i . \hat{n}_i <0$).
The node features $\phi_n(i)$
consist of visual appearance features based on histogram of HSV values and the histogram of gradients
(HOG), as well as local shape and geometry features that capture properties such as how planar
a segment is, its absolute location above ground, and its shape. Some features capture
spatial location of an object in the scene (e.g.,  N9).
%  captures the tendency of some objects to be near the walls). 

We connect two segments (nodes) $i$ and $j$ by an edge if there exists a point in segment $i$ and 
a point in segment $j$ which are less than \emph{context\_range} distance apart. This captures the
closest distance between two segments (as compared to centroid distance between the segments)---we 
study the effect of context range more in Section~\ref{sec:experiments}.
The edge features $\phi_t(i,j)$ (Table \ref{tab:Features}-right) consist of associative features (E1-E2)
based on visual appearance and local shape, as well as non-associative features (E3-E8) that capture
the tendencies of two objects to occur in certain configurations.
%  (see Section \ref{S.properties}).
% For example, E9 is positive if segment $i$ is in front of segment $j$ and negative otherwise
% (see Fig.~\ref{}).

Note that our features are insensitive to horizontal translation and 
rotation of the camera. However, our features place a lot of emphasis on the vertical direction 
because gravity influences the shape and relative positions of objects to a large extent.

% put eqatuins in a separate line for ease in commenting out
\begin{table}[t!]
\vskip -.15in
{\scriptsize
\begin{minipage}[b]{6cm}\centering

\begin{tabular}{|p{5.0cm}|c|}
\multicolumn {2}{c}{Node features for segment $i$.} \\ 
\hline 
 Description  & Count\\ \hline
{\bf Visual Appearance} & {\bf 48} \\
N1. Histogram of HSV color values & 14 \\
N2. Average HSV color values & 3 \\
N3. Average of HOG features of the blocks in image spanned by the points of a segment & 31 \\
\hline
{\bf Local Shape and Geometry} & {\bf 8} \\
N4. linearness (${\lambda_{i0}}$ - ${\lambda_{i1}}$), planarness (${\lambda_{i1}}$ - ${\lambda_{i2}}$) & 2 \\
% N5. & 1 \\ 
N5. Scatter: ${\lambda_i}_0$ & 1 \\ 
N6. Vertical component of the normal: ${\hat{n_i}}_z$ & 1 \\ 
N7. Vertical position of centroid: ${c_i}_z$ & 1 \\ 
N8. Vert.~and Hor.~extent of bounding box  & 2 \\ 
% N10. Horizontal extent of bounding box  & 1 \\ 
N9. Dist.~from the scene boundary (Fig.~\ref{fig:features})& 1 \\
\hline
\end{tabular}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}[b]{6cm}
\centering
\begin{tabular}{|p{5.7cm}|c|}
\multicolumn {2}{c}{Edge features for (segment $i$, segment $j$).}\\ \hline
 Description  & Count\\ \hline
{\bf Visual Appearance (associative)} & {\bf 3} \\
E1. Difference of avg HSV color values & 3\\
\hline
{\bf Local Shape and Geometry (associative)} & {\bf 2} \\
E2. Coplanarity and convexity (Fig.~\ref{fig:features})
& 2\\ 
\hline
{\bf Geometric context (non-associative)} & {\bf 6} \\

E3. Horizontal distance b/w centroids.
% $\sqrt{({c_i}_x - {c_j}_x)^2 + ({c_i}_y - {c_j}_y)^2 }$ 
& 1\\ 

E4. Vertical Displacement b/w centroids:
 $(c_{iz} - c_{jz})$ 
& 1\\ 

E5. Angle between normals (Dot product):
$ \hat{n}_i \cdot \hat{n}_j $
& 1\\ 

E6. Diff.~in angle with vert.:
$ \cos^{-1}({n_{iz}})$ - $\cos^{-1}({n_{jz}}) $
& 1\\

E8. Dist.~between closest points:
$ \min_{u\in s_i,v\in s_j} d(u,v) $ (Fig.~\ref{fig:features})
& 1\\
 
E8. rel.~position from camera (in front of/behind).
% $ |rh_i|_2 - |rh_j|_2 $ 
(Fig.~\ref{fig:features})
& 1\\ 

\hline

\end{tabular}

\end{minipage}
}
\vspace*{\captionReduceTop}
\caption{{\small Node and edge features.} }
\label{tab:Features}
\vspace*{\captionReduceBot}
\end{table}

\fi

% All point-clouds are aligned so that the z-axis is always vertical and the ground is at zero height. It's reasonabe to assume that the robot knows the height and orientation of it's kinect sensor.  
% Also, there is no ambiguity of scale in the input pointcould and all distance mearurements are in metres. Here, we describe some of the non-trivial features.
% N11 (see table) captures the tendency of some objects to be near the walls. 
% E1, E2 and E3 capture the tendency of connected segments to be a part of the same object.
% E4 and onwards can capture the tendency of different objects to occur in certain configurations(see Geometrical Context in section \ref{S.properties}). E9 is positive if segment i is infront of segment j and negative otherwise. 

% NExT LINE ALREADY COVERED IN MODELS SECTION
%For every segment we compute a set of features which describe their visual and shape properties.We call these the node features.  
\begin{comment}
\begin{table}[!h]

          \begin{center}
            \begin{tabular}{|c|c|c|c|} \hline

                \multicolumn {2}{|c|}{Node Features  }  &   \multicolumn {2}{|c|}{Edge features }\\ \hline
               Description  & Count& Description  & Count\\ \hline
                                linearness : ${\lambda}_0$ & 1 & horizontal distance b/w centroids $\sqrt{(x_{ci} - x_{cj})^2 + (y_{ci} - y_{cj})^2 }$ & 1 \\             
            \end{tabular}
         \caption{Description of features}
         \label{tab:potentialsEffect}
        \end{center} 
\end{table}
\end{comment}


% \todo{Feature figures can perhaps go here....}



%
%\label{fig:inFrontOf}
%\end{minipage}
%\hspace{0.1cm}
%\begin{minipage}[b]{0.3\linewidth}
%\centering
%\includegraphics[scale=0.4]{normalpc.pdf}
%\label{fig:convexity}
%\end{minipage}
%\hspace{0.1cm}
%\begin{minipage}[b]{0.3\linewidth}
%\centering
%\includegraphics[scale=0.35]{mindist.pdf}
%\label{fig:mindist}
%\end{minipage}

\begin{comment}
\begin{packed_item}


\item linearness, planarity and scatterness of the segment: These are the geometric features commonly used in the spectral analysis of point clouds. if $\lambda_2 \ge \lambda_1 \ge lambda_0 $ are the first three Eigen values of the scatter matrix $M$ defined over the points of a segment, the linearness, planarity and scatterness are given by $\lambda_2 - \lambda_1$,  $\lambda_2 - \lambda_1$ and $\lambda_0$ respectively.
\item histogram of color values in HSV space
\item vertical component of the normal
\item vertical position of the centroid: i.e., the height of centroid from the ground
\item vertical and horizontal size of Bounding box: Given the dimensions of the bounding box of a segment $(length,width,height)$ , the vertical size given by $height$ and the horizontal size is measured as $\sqrt{ length^2 \times width^2}$
\item distance from the point cloud boundary

\end{packed_item}

If there are 2 points lying in different segments and are less than  {\it min\_edge\_dist} apart, they are connected by an edge in our graph. We report performances on 3 values of {\it min\_edge\_dist} : 30cm,60cm,120cm.
For pairs of segments, $s_i$ and $s_j$,  connected by an edge, we compute the following edge features:
Let $ \overrightarrow{c_i} = (x_{ci},y_{ci},z_{ci})$ be the centroid of segment $s_i$ and $ \overrightarrow{c_j} = (x_{cj},y_{cj},z_{cj})$ be the centroid of segment $s_j$ and and let $ \overrightarrow{n_i}$ and $ \overrightarrow{n_j}$ are the normals of segment $s_i$ and $s_j$ respectively. 
\begin{packed_item}
\item horizontal distance between centroids: $\sqrt{(x_{ci} - x_{cj})^2 + (y_{ci} - y_{cj})^2 }$ 
\item vertical displacement between centroids: $z_{ci} - z_{cj}$
\item dot product between normals: $ \hat{n}_i \cdot \hat{n}_j $
\item difference in distance from camera location(is a segment infront of another?)
\item Coplanarity: Coplanarity is defined  as follows:\\
\[
Coplanarity(s_i,s_j) = \left\{
  \begin{array}{l l}
    -1 & \quad  \hat{n}_i \cdot \hat{n}_j \le \cos{\alpha}  \\
    1/d_{ij} & \quad \mbox{otherwise} \\
  \end{array} \right. 
\] 
, where $d_{ij} = abs(( \overrightarrow{c_i} - \overrightarrow{c_j}) \cdot  \hat{n_i}  )$ is the distance between centroids in the direction of the normals and $\alpha$ is the tolerance angle.
\item Convexity: This feature determines if the two adjoined segments form a convex surface and is defined as: \\
\[
Convexity(s_i,s_j) = \left\{
  \begin{array}{l l}
    1 & \quad  (md_{ij} < \tau) \wedge [ [ ( \hat{n}_i \cdot   \overrightarrow{d_{ij}} \le 0 )   \wedge   ( \hat{n}_j \cdot   \overrightarrow{d_{ji}} \le 0) ] \vee \hat{n}_i \cdot \hat{n}_j \le \cos{ \alpha} ]  \\ 
    0 & \quad \mbox{otherwise}\\
  \end{array} \right.
  \]
 where  $md_{ij}$ is the minimum distance between segments $s_i$ and $s_j$, $\overrightarrow{d_{ij}} = (\overrightarrow{c_j}  - \overrightarrow{c_i} )$, is the displacement vector from  $\overrightarrow{c_i}$  to  $\overrightarrow{c_j}$  and 
 $\overrightarrow{d_{ji}} =  - \overrightarrow{d_{ij}} $.  $\tau$ and $\alpha$ are the tolerance values for minimum distance and the angle respectively.
\end{packed_item}
\end{comment}

% \todo{Would need some more details, and clear mathematical description here. See recent paper on placing
% objects by Yun for this. Write the features section properly as she did.}

\begin {comment} 
\vspace*{\subsectionReduceTop}
\subsection{Relative Features}
\vspace*{\subsectionReduceBot}

\todo{This section describes the relative features in more detail.}

We model the following geometric relations between a pair of
 segments:  relative depth-ordering, relative horizontal-ordering, coplanar-ness, etc.  
For any given pair of segments, the relative depth-ordering  captures the ``infront-of", ``behind" and 
``none" relations and the relative  horizontal-ordering captures the ``above", ``below" and ``same height" relations.
\end{comment}


==> preliminaries.tex <==
%evspace*{\sectionReduceTop} 
\section{Scene Grammar}
%\vspace*{\sectionReduceBot}
\label{sec:SceneGrammar}
Our Scene Grammar is a five-tuple $G = (S,V,R,f,g)$. 
S is the start symbol which represents the whole scene(root of the parse-tree)root of the parse-tree. 
$V=V^N \cup V^T$, where $V^T$ represents the set of terminal nodes. 
There are the planar segments generated by oversegmenting the 3D pointcloud given as input. 
%So, $V^T=\{segment\}$.
Multiple segments may belong to the same part of an object.
$V^N$ are the non-terminal nodes which are obtained by combining terminals(e.g. Plane, Table, TableTop).
%Each symbol in $V$ is associated with a a vector of features $x \in R^d$.
R is the set of production-rule schemas which combine a string of terminals and non-terminals to form a non-terminal. 

Here are few examples: \\
\begin{enumerate}
\item Plane $->$ segment\\
\item Plane $->$ Plane segment\\
\item TableTop $->$  Plane\\
\item Table  $->$ TableTop TableLegLeft TableLegRight\\
\item Table  $->$ TableTop TableLegLeft TableLegRight TableDrawer\\
\end{enumerate}

Rules 2 can be used to recursively combine multiple segments into a plane.
Rules 3 and 4 show how we can capture structural variation in Tables(some tables can have a drawer).
The rules like those mentioned above compose segments into planes, form object-parts from planes, and objects from object-parts
To capture relationships between objects, we add the following rules:

\begin{enumerate}
\setcounter{enumi}{5}
\item TableComplex  $->$ Table\\
\item TableComplex  $->$ TableComplex Monitor\\
\item TableComplex  $->$ TableComplex CPU\\
\item TableComplex  $->$ TableComplex Keyboard\\
\end{enumerate}

For an object X, we call XComplex as an entity containing X and all objects placed on it.
Rule 6 forms a TableComplex out of a Table and rules 7-9 recursively add other tabletop-objects to it.
Finally, we have the following rule for the start symbol(which represents the whole scene):


\begin{enumerate}
\setcounter{enumi}{9}
\item S $->$ FloorComplex
\end{enumerate}

The full list of rules can be found in Supplementary Material.
The function $f$ takes a set $s \in V$  and and returns the corresponding features as a vector of real numbers. These features contain both the features dependent on individual nodes
and the relative features between pairs of nodes in $s$. For example, for a Plane p, f(p) contains it's normal direction, position of centroid and area of convex hull.
For a TableTop tp and a TableLeg tl, f(tp,tl) contains relative features like signed difference between the z coordinates of highest point in tl and lowest point in tp. 
We will talk more about features in secion \ref{sec:Features}. 
The function g computes the score of applying a rule $r$ to a set of nodes $s$. Intuitively, $s$ contains nodes corresponding to the symbols in RHS of the rule r.
We consider the following forms of $g$
\begin{eqnarray}
g_{nb}(r,s)&=&w^T f(s)\\
g_{nb}(r,s)&=&w^T f(s) 
\end{eqnarray}


